OneAdapt: Adaptive Compilation for Resource-Constrained Photonic One-Way Quantum Computing

Measurement-based quantum computing (MBQC), a.k.a. one-way quantum computing (1WQC), is a universal quantum computing model, which is particularly well-suited for photonic platforms. In this model, computation is driven by measurements on an entangled state, which serves as an intermediate representation (IR) between program and hardware. However, compilers on previous IRs lacks the adaptability to the resource constraint in photonic quantum computers. In this work, we propose a novel IR with new optimization passes. Based on this, it realizes a resource-adaptive compiler that minimizes the required hardware size and execution time while restricting the requirement for fusion devices within an adaptive limit. Moreover, our optimization can be integrated with Quantum Error Correction (QEC) to improve the efficiency of photonic fault-tolerant quantum computing (FTQC).

==> 07_compilation_time_eval.tex <==
\begin{table*}[hb]
    \centering
      \caption{\revise{Compilation time and 1D depth varying with $p$.}}
      % \vspace{-5pt}
      
    \resizebox{0.96\linewidth}{!}{
        \renewcommand*{\arraystretch}{1}
        \begin{small}
            \begin{tabular}{|p{0.7cm}|p{1.5cm}|p{1.5cm}|p{1cm}|p{0.9cm}|p{1.6cm}|p{1.5cm}|p{0.9cm}|p{1.8cm}|p{1.8cm}|p{0.9cm}|}
        
        \hline
        $p$  & Benchmark -\#Qubit & OnePerc 1D Depth & Our 1D Depth  & Improv. & OnePerc Runtime (s/layer) & Our Runtime (s/layer) & Improv. & OnePerc Offline Comp. Time (s) & Our Offline $\quad$ Comp. Time (s)  & Improv.\\
        \hline
        \multicolumn{1}{|c|}{\multirow{4}{*}{\parbox{2cm}{ 0.1 }}}
        & QAOA-36 & 1,653 & 579 & 2.85 & 0.14 & 0.13 & 1.09 & 18.14 & 13.19 & 1.38 \\
        \cline{2-11}
        & QFT-36 & 4,531 & 1,364 & 3.32 & 0.14 & 0.14 & 1.02 & 163.47 & 101.42 & 1.61 \\
        \cline{2-11}
        & RCA-36 & 2,547 & 2,502 & 1.02 & 0.15 & 0.12 & 1.28 & 65.71 & 65.29 & 1.01 \\
        \cline{2-11}
        & VQE-36 & 1,243 & 472 & 2.63 & 0.14 & 0.14 & 1.03 & 16.13 & 10.74 & 1.5 \\
        \hline
        \multicolumn{1}{|c|}{\multirow{4}{*}{\parbox{2cm}{ 0.2 }}}
        & QAOA-36 & 1,653 & 459 & 3.6 & 0.14 & 0.14 & 0.99 & 18.14 & 10.7 & 1.7 \\
        \cline{2-11}
        & QFT-36 & 4,531 & 1,130 & 4.01 & 0.14 & 0.15 & 0.93 & 163.47 & 87.15 & 1.88 \\
        \cline{2-11}
        & RCA-36 & 2,547 & 1,750 & 1.46 & 0.15 & 0.13 & 1.14 & 65.71 & 47.14 & 1.39 \\
        \cline{2-11}
        & VQE-36 & 1,243 & 346 & 3.59 & 0.14 & 0.15 & 0.93 & 16.13 & 9.24 & 1.75 \\
        \hline
        \multicolumn{1}{|c|}{\multirow{4}{*}{\parbox{2cm}{ 0.4 }}}
        & QAOA-36 & 1,653 & 388 & 4.26 & 0.14 & 0.17 & 0.82 & 18.14 & 9.95 & 1.82 \\
        \cline{2-11}
        & QFT-36 & 4,531 & 946 & 4.79 & 0.14 & 0.18 & 0.78 & 163.47 & 73.98 & 2.21 \\
        \cline{2-11}
        & RCA-36 & 2,547 & 1,271 & 2.0 & 0.15 & 0.18 & 0.85 & 65.71 & 36.74 & 1.79 \\
        \cline{2-11}
        & VQE-36 & 1,243 & 289 & 4.3 & 0.14 & 0.19 & 0.75 & 16.13 & 7.95 & 2.03 \\
        \hline
        
        \end{tabular}
        \end{small}
    }
    \label{tab:varying_p}
\end{table*}

\subsection{\revise{Compilation Time}}
\revise{\textbf{Runtime Overhead} While frequent node refreshes can reduce the 1D depth, it may also increase the runtime overhead due to the denser temporal edges generated by those refresh. This can be balanced by adjusting the frequency of non-mandatory node refresh, through the parameter $p$ in equation~\ref{parameter_p} of Section~\ref{sect:dynamic_refreshing}. We demonstrate this tradeoff by varying $p$ from 0.1 to 0.4 for compiling 36-qubit programs onto an IR of \retodo{$4\times4$} 2D size, renormalized from \retodo{$96\times 96$} RSLs with a fusion success probability of \retodo{75\%}, which are consistent to the evaluataion setting of OnePerc. Table~\ref{tab:varying_p} shows the 1D depth and the average runtime overhead per RSL. Note that the absolute values are not important as we implemented the codes in python.  It can be seen that when $p=0.2$, our framework achieves a significant 1D depth improvement of \retodo{3.17}, with a similar runtime overhead with OnePerc.
If allowed for more runtime, the 1D depth improvement can also be increased by increasing $p$.}


\revise{\textbf{Offline Compilation}
% As shown in Fig.~\ref{fig:offline_time}, the offline compilation time of our framework increases with the program size (programs are compiled to their \retodo{standard 2D sizes}). Moreover, 
Our compiler exhibits a shorter compilation time than OnePerc,
primarily because its reduction in 1D depth reduces the number of layers that the compiler needs to search. As shown in Table~\ref{tab:varying_p}, for 36-qubit programs on \retodo{$4\times4$} 2D size of IR, our framework reduces the offline compilation by an average factor of \retodo{1.67}. Both the 1D depth and offline compilation time increase with a more frequent node refresh (an increased $p$).}

